Draft, Sketch, and Prove: Guiding Formal Theorem Provers with Informal Proofs

The formalization of existing mathematical proofs is a notoriously difficult process. Despite decades of research on automation and proof assistants, writing formal proofs remains arduous and only accessible to a few experts. While previous studies to automate formalization focused on powerful search algorithms, no attempts were made to take advantage of available informal proofs. In this work, we introduce Draft, Sketch, and Prove (DSP), a method that maps informal proofs to formal proof sketches, and uses the sketches to guide an automated prover by directing its search to easier sub-problems. We investigate two relevant setups where informal proofs are either written by humans or generated by a language model. Our experiments and ablation studies show that large language models are able to produce well-structured formal sketches that follow the same reasoning steps as the informal proofs. Guiding an automated prover with these sketches enhances its performance from 20.9% to 39.3% on a collection of mathematical competition problems.

==> figures/algorithm.tex <==

\begin{figure}[ht]
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State {\bf Inputs:}\\
\quad \quad Informal statement~(IS), Formal statement~(FS), Autoformalization examples~(AE)
\State {\bf Output:}\\
\quad \quad Valid Isabelle proof or None
\For{n\_informal\_proofs}
\State Informal proof draft~(IPD) $\gets$ \texttt{Human}~(IS) or \texttt{Language model}~(IS)
\For{n\_proof\_sketches}
\State Formal proof sketch~(FPS) $\gets$ Sample from \texttt{Autoformalizer}~(AE, IS, IPD, FS)
\ForAll{gap $\in$ FPS}
\State FPS $\gets$ FPS~[\texttt{Prover}~(gap) / gap]
\EndFor
\If{FPS is a valid proof to FS}
\State \Return FPS
% \Else
% \State \Return None
\EndIf
\EndFor
\EndFor
\end{algorithmic}
\caption{Draft, Sketch, and Prove}
\label{alg}
\end{algorithm}
\end{figure}


==> figures/proof_example.tex <==
\begin{figure}[t]
%\begin{figure}
\begin{tcolorbox}[colback=mybrown!5!white,colframe=mybrown!75!black]
\begin{small}
\textbf{Statement:}
Show that for any prime $p$ and any integer $n$, we have $p \mid n$ if and only if $n^2 \equiv 0 \pmod{p}$.
\Sepline
\textbf{Informal Proof (Minerva 62B):}\\
Suppose $p \mid n$. Then $n = pk$ for some $k$, and $n^2 = (pk)^2 = p^2k^2 = 0 \pmod{p}$. \\
Conversely, suppose $n^2 \equiv 0 \pmod{p}$. Then $p \mid n^2$, and hence $p \mid n$, since $p$ is prime.
\Sepline
\textbf{Formal Proof:}
\vspace{-1.5em}
\begin{lstlisting}[style=isabelle]
theorem numbertheory_prmdvsneqnsqmodpeq0:
  fixes n :: int and p :: nat 
  assumes "prime p" 
  shows "p dvd n $\mathbf{\longleftrightarrow}$ (n^2) mod p = 0"
proof - 
(* Suppose $\mathbf{\textcolor{red}{p \mid n}}$. Then $\mathbf{\textcolor{red}{n = pk}}$ for some $\mathbf{\textcolor{red}{k}}$, and $\mathbf{\textcolor{red}{n^2 = (pk)^2 = p^2k^2 = 0 \pmod{p}}}$. *)
$\mathbf{\textcolor{isarblue}{\{}}$ assume c0: "p dvd n" obtain k :: int where c1: "n = p * k" using c0 
    by auto [ATP]
  hence "(n^2) mod p = (p^2 * k^2) mod p" using c0 
    by (auto simp: field_simps) [ATP]
  also have "\<dots> = 0" using c0 
    by auto  [ATP]
  finally have "(n^2) mod p = 0" using c1 
    by auto  [ATP]
$\mathbf{\textcolor{isarblue}{\}}}$ moreover 
$\mathbf{\textcolor{isarblue}{\{}}$ assume c0: "(n^2) mod p = 0" have "p dvd n^2" using c0 
    by auto  [ATP]
  hence "p dvd n" using assms 
    by (smt (z3) dvd_0_right power_eq_0_iff prime_nat_int_transfer
        prime_dvd_power_int prime_dvd_power) [ATP]
$\mathbf{\textcolor{isarblue}{\}}}$ ultimately show ?thesis
    by auto  [ATP]
qed
\end{lstlisting}
\end{small}
\end{tcolorbox}
\caption{
\small
\textbf{A successful formal proof synthesized with an informal proof generated by a language model.} The Minerva~($62$B) model generates a correct informal proof to a problem which guides the automated prover to a formal proof.
The formal proof aligns with the informal proof and verifies the implications in both directions.
}
\label{fig:example_iff}
\end{figure}

==> lstisabelle.tex <==
% Not really meant for highlighting isabelle source, but for easily writing latex that looks like
% isabelle
% 
% keyword level 1 - isabelle outer syntax 
% keyword level 2 - isabelle inner syntax programming constructs (if, let, etc)
% keyword level 3 - standard constants (length, mod, etc)
% keyword level 4 - isabelle proof methods


% \newcommand{\lsem}{\ensuremath{\mathopen{[\![}}}
% \newcommand{\rsem}{\ensuremath{\mathclose{]\!]}}}

\lstdefinelanguage{isabelle}{
  morekeywords={theorem,theorems,corollary,lemma,lemmas,locale,begin,end,fixes,assumes,shows,and,class,
    constrains , definition, where, apply, done,unfolding, primrec, fun, using, by, for, uses, file,
    schematic_lemma, concrete_definition, prepare_code_thms, export_code, datatype, type_synonym, typedef, value,
    proof, next, qed, show, have, hence, thus, interpretation, fix, context, sepref_definition,sepref_def,is,export_llvm
 } ,
  morekeywords=[2]{rec, return, bind, foreach, if, then, else, do, let, in, res, spec, fail, assert, while, case, of, 
    check, get, set},
%  morekeywords=[3]{length,mod,insert},
%   morekeywords=[4]{simp,auto,intro,elim,rprems,refine_mono,refine_rcg},
  sensitive=True,
  morecomment=[s]{(\*}{\*)},
}


\DeclareTextCommand{\shortunderscore}{T1}{%
  \leavevmode \kern.06em\vbox{\hrule width.4em}}

\renewcommand{\textunderscore}{\shortunderscore}  
  
\lstset{
    language=isabelle,
    mathescape=true,
    escapeinside={--"}{"},
    basicstyle={\itshape},
    keywordstyle=\rm\ttfamily\fontseries{b}\selectfont,
    keywordstyle=[2]\rm\ttfamily\fontseries{m}\selectfont,
    keywordstyle=[3]\rm,
    keywordstyle=[4]\rm,
    showstringspaces=false,
    keepspaces=true,
    columns=[c]fullflexible}
\lstset{literate=
  {"}{}0
  {'}{{${}^\prime\!$}}1
  {\%}{{$\lambda$}}1
  {\\\%}{{$\lambda$}}1
  {\\\$}{{$\mathbin{\,\$\,}$}}1
  {->}{{$\rightarrow$}}1
  {<-}{{$\leftarrow$}}1
  {<.}{{$\langle$}}1
  {.>}{{$\rangle$}}1
  {<=}{{$\le$}}1
  {>=}{{$\ge$}}1
  {<->}{{$\leftrightarrow$}}1
  {-->}{{$\longrightarrow$}}2
  {<-->}{{$\longleftrightarrow$}}1
  {=>}{{$\Rightarrow$}}1
  {==}{{$\equiv$}}2
  {==>}{{$\implies$}}2
  {<=>}{{$\Leftrightarrow$}}1
  {~=}{{$\ne$}}1
  {|}{{$\mid$}}1
  {-`}{{$\rightharpoonup$}}1
  {|`}{{$\restriction$}}1
  {!!}{{$\bigwedge$}}1
  {(}{{$($}}1
  {)}{{$)$}}1
  {\{}{{$\{$}}1
  {\}}{{$\}$}}1
  {[}{{$[$}}1
  {]}{{$]$}}1
  {[|}{{$\llbracket$}}1
  {|]}{{$\rrbracket$}}1
  {\\<lbrakk>}{{$\lsem$}}1
  {\\<rbrakk>}{{$\rsem$}}1
  {|-}{{$\vdash$}}1
  {|=}{{$\models$}}1
  {|->}{{$\mapsto$}}1
  {|_|}{{$\bigsqcup$}}1
  {...}{{$\dots$}}1
  {\\x}{{$\times$}}1
  {_0}{{${}_0$}}1
  {_1}{{${}_1$}}1
  {_2}{{${}_2$}}1
  {_3}{{${}_3$}}1
  {_4}{{${}_4$}}1
  {_5}{{${}_5$}}1
  {_6}{{${}_6$}}1
  {_7}{{${}_7$}}1
  {_8}{{${}_8$}}1
  {_9}{{${}_9$}}1
  {_L}{{${}_L$}}1
  {\\_n}{{${}_n$}}1
  {\\_i}{{${}_i$}}1
  {\\_j}{{${}_j$}}1
  {\\_x}{{${}_x$}}1
  {\\_y}{{${}_y$}}1
  {\\impl}{{${}_\dagger$}}1
  {^*}{{$^*$}}1
  {^k}{{$^k$}}1
  {^d}{{$^d$}}1
  {\\<^sup>*}{{$^*$}}1
  {\\<^sub>*}{{$_*$}}1
  {\\<^sub>A}{{$_A$}}1
  {\\<^sub>r}{{$_r$}}1
  {\\<^sub>a}{{$_a$}}1
  {:_i}{{$:_i$}}1
  {\\<A>}{{$\mathcal{A}$}}1
  {\\<O>}{{\sf o}}1
  {\\<Phi>}{{$\Phi$}}1
  {\\<Psi>}{{$\Psi$}}1
  {\\<sigma>}{{$\sigma$}}1
  {\\<cdot>}{{$\cdot$}}1
  {\\<in>}{{$\in$}}1
  {\\<le>}{{$\le$}}1
  {\\<noteq>}{{$\ne$}}1
  {\\<lambda>}{{$\lambda$}}1
  {\\<longrightarrow>}{{$\longrightarrow$}}1
  {\\<longleftrightarrow>}{{$\longleftrightarrow$}}1
  {\\<Rightarrow>}{{$\Rightarrow$}}1
  {\\<Longrightarrow>}{{$\Longrightarrow$}}1
  {\\<rightarrow>}{{$\rightarrow$}}1
  {\\<leftarrow>}{{$\leftarrow$}}1
  {\\<mapsto>}{{$\mapsto$}}1
  {\\<equiv>}{{$\equiv$}}1
  {\\<and>}{{$\wedge$}}1
  {\\<or>}{{$\vee$}}1
  {\\<And>}{{$\bigwedge$}}1
  {\\<Up>}{{$\Uparrow$}}1
  {\\<Down>}{{$\Downarrow$}}1
  {\\<Union>}{{$\bigcup$}}1
  {\\<up>}{{$\uparrow$}}1
  {\\<down>}{{$\downarrow$}}1
  {\\<times>}{{$\times$}}1
  {\\<forall>}{{$\forall$}}1
  {\\<exists>}{{$\exists$}}1
  {\\<nexists>}{{$\nexists$}}1
  {\\<union>}{{$\cup$}}1
  {\\<inter>}{{$\cap$}}1
  {\\<subset>}{{$\subset$}}1
  {\\<subseteq>}{{$\subseteq$}}1
  {\\<supset>}{{$\supset$}}1
  {\\<supseteq>}{{$\supseteq$}}1
  {\\<alpha>}{{$\alpha$}}1
  {\\<beta>}{{$\beta$}}1
  {\\<gamma>}{{$\gamma$}}1
  {\\alpha}{{$\alpha$}}1
  {\\beta}{{$\beta$}}1
  {\\gamma}{{$\gamma$}}1
  {\\<Gamma>}{{$\Gamma$}}1
  {\\<langle>}{{$\langle$}}1
  {\\<rangle>}{{$\rangle$}}1
  {\\<not>}{{$\neg$}}1
  {\\<box>}{{$\oblong$}}1
  {\\<bot>}{{$\bot$}}1
  {\\<top>}{{$\top$}}1
  {\\<notin>}{{$\notin$}}1
  {\\<guillemotright>}{{$\gg$}}1
  {\\in}{$\in$}1
  {\\and}{$\wedge$}1
  {\\or}{$\vee$}1
  {\\Phi}{{$\Phi$}}1
  {\\Psi}{{$\Psi$}}1
  {\\le}{{$\le$}}1
  {\\Up}{{$\Uparrow$}}1
  {\\Down}{{$\Down$}}1
  {>>}{{$\gg$}}1
  {>>=}{{${\gg}{=}$}}1
  {<*lex*>}{{$\times_{\sf lex}$}}1
  {\\<open>}{{\rm\guilsinglleft}}1
  {\\<close>}{{\rm\guilsinglright}}1
}

% % \newcommand{\is}{\lstinline[language=isabelle,basicstyle=\normalsize\ttfamily\slshape]}
% \newcommand{\is}{\lstinline[language=isabelle]}
% \newcommand{\q}[1]{\mbox{\guilsinglleft{#1}\hspace{-.0pt}\guilsinglright}}
% % \newcommand{\isai}[1]{\q{\lstinline[language=isabelle,basicstyle=\normalsize\ttfamily\slshape]{#1}}}
% \cMakeRobust\q

==> sections/formatting.tex <==

\section{Submission of conference papers to ICLR 2023}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/one_page.tex <==
\newpage
\section*{One-page summary of the paper}

\subsection*{Abstract}
People often take inspiration from textbook mathematical proofs to formally express them in interactive theorem provers.
However, the automation of formal proofs has not been able to leverage their informal counterparts, despite that they often reveal the structures, if not the entirety of proofs. Our paper presents a novel approach to overcome this limitation. Concretely, we use informal solvers (humans or state-of-the-art language models) to obtain informal proofs. Then we use in-context learning with large language models to generate formal proof sketches. Finally, automated theorem provers are deployed to complete the sketches into full proofs. 
With human-written informal proofs and language-model-generated informal proofs, we successfully prove $37.3\%$ and \todo{x}$\$$ of problems respectively, on a collection of high-school competition problems. This method expands the modes of mathematical data that can be automatically formalised and can be facilitating to the formalisation procedure.

\subsection*{Introduction}
\begin{itemize}
    \item Informal proofs provide guidance for formal proof writing but automated theorem provers have not been able to utilize them effectively.
    \item This paper overcomes this limitation. We use informal solvers to come up with informal proofs to problems, and then use large language models to translate the informal proofs into formal ones that can be checked and verified.
    \item Contributions: (1) A dataset of high school competition problems with aligned tuples of (informal statement, informal proof, formal statement); (2) A novel framework that generates formal proofs by leveraging informal counterparts; (3) Techniques for improving the performance of autoformalizing proof sketches and corresponding ablation studies.
\end{itemize}
\subsection*{Background}
\begin{itemize}
    \item Informal proofs and formal proofs, comparison. Abundant but not grounded vs computer-understandable but very scarce.
    \item Sledgehammer.
\end{itemize}
\subsection*{Related works}
\begin{itemize}
    \item ML approaches to formal theorem proving
    \item ML approaches to informal theorem proving
    \item Autoformalization
\end{itemize}
\subsection*{Method}
\begin{itemize}
    \item In-context learning\\
    The amount of parallel informal-formal proof data is very small. Therefore the translation between them is difficult for standard machine translation methods. There are ways to deal with such situations (e.g. unsupervised translation (cite some of guillaume's earlier work)). For this paper we decide to use in-context learning, i.e. use demonstrations of input/output pairs to induce algorithmic behavior accomplishing the task. Discussion on this in detail.
    \item Proof skeleton/sketch\\
    We want to align the informal and formal proofs for the autoformalization. However the formal proofs can often contain steps that are not present in informal ones~(those with metis etc.). This presents a challenge for the alignment. To deal with it we abstract away such steps with sledgehammer (cite thor's idea).
    
\end{itemize}
\subsection*{Experiments}
Baselines
\begin{itemize}
    \item Sledgehammer on MiniF2F: $10\%$
    \item Sledgehammer + heuristics on MiniF2F: $20\%$
    \item Codex + formal statement -> formal proof sketch
    \item Codex + informal statement + formal statement -> formal proof sketch
\end{itemize}
Results
\begin{itemize}
    \item Codex + informal statement + human informal proof + formal statement -> formal proof sketch
    \item Codex + informal statement -> codex informal proof;\\
    Codex + informal statement + codex informal proof + formal statement -> formal proof sketch
    \item Minerva + informal statement -> Minerva informal proof;\\
    Codex + informal statement + minerva informal proof + formal statement -> formal proof sketch
\end{itemize}
Ablations
\begin{itemize}
    \item The use of inline comments
    \item The use of sampling temperature
    \item The use of number of examples in prompts
\end{itemize}
\subsection*{Conclusion}
\begin{itemize}
    \item We showed the benefit and the feasibility of leveraging informal proof for formal proof generation.
    \item Future work: use better off-the-shelf prover than Sledgehammer to solve intermediate goals.
\end{itemize}
\newpage





==> tmp.tex <==

%%% TIM

% % The automated writing of formal interactive proofs is a challenging task that has been the focus of increased attention in recent years \citep{}. Tackled with large language models, this task provides quantitative insights into their reasoning capabilities without the cost of manual verification which is necessary in the informal setting. 
% % Despite interesting early results where language models are coupled with search methods, the automated proving capabilities of these systems seems to lag behind the informal results obtained with large language models in \citet{Minerva}.

% % Whereas informal mathematical data is abundant enough to fine-tune a large language model, formalised proofs are scarce as they can only be written by a few experts. In this work, we explore two avenues to leverage informal data for the goal of producing formal proofs. Our methods hinge on so called proof-sketches, which are high level sequences of reasoning steps written in a formal language, where each step is expected to be amenable to automatic proving. In this work, we focus on the Isabelle language and its powerful Sledgehammer for solving these intermediate steps. An example proof sketch is provided in Figure~\ref{fig:proof_skeleton}.

%%% GUI

% The application of machine learning methods to symbolic reasoning has been the focus of increased attention in the past few years.
% But in spite of promising results, the applications of deep learning to automated theorem proving were not as successful as in other domains.
% Large neural networks thrive when data is abundant, but are also prone to overfit when data is scarce, and the small amount of existing formalized mathematics has hindered the successes of deep models in that field.
% The annotation process being particularly labor-intensive, and only accessible by a handful of human specialists, generating large datasets of formalized mathematics is also not realistic.
% As a result, previous studies have instead relied on large scale pretraining~\cite{polu,htps}, the use of auxiliary tasks to improve generalization~\cite{PACT}, or to use reinforcement learning or expert iteration to augment the dataset of human proofs with successful trajectories~\cite{}.

% Unlike formalized mathematical data, informal data is abundant and widely available online. 
% In particular, large language models trained on a massive amount of math web pages recently showcased impressive reasoning abilities~\cite{minerva}.
% In this paper, we investigate a new setting where we leverage informal proofs (e.g. a proof written in Latex) to guide an automated theorem prover, by generating a formal \textit{proof sketch} with intermediate subgoals that follow the same reasoning steps as the informal proof (\autoref{fig:summary}).
% Intuitively, the proof sketch captures the global argument structure, reducing the proof to filling in local gaps.
% Our key idea is to use large-scale language models to generate these  proof sketches based on informal proofs,  offloading the task of filling in the gaps to a separate specialized system.
% % An example of informal proof with its corresponding proof skeleton is provided in Figure~\ref{fig:proof_skeleton}.

% We study two different settings. First, we consider that the informal proofs of the statements to prove are given and are valid human proofs.
% This is an interesting setting as the formalization of existing mathematical textbooks is already an expensive and tedious process, although proofs are available.
% Second, we generate informal proofs using a large language models.
% Although generated proofs might be erroneous, they can still contain relevant intermediate subgoals likely to help an automated prover.



%%%%%%%%%
% say that formal proving is hard / tedious ?
% however, not as successful in formal proving where data is tiny
% however, deep learning its great when lots of data
% annotation is hard so people do X and Y
The automated writing of formal proofs is a challenging task that has been the focus of increased attention in recent years \citep{}.
However, deep-learning approaches have not proved as successful as in other domains, such as vision or natural language processing, where data is abundant. 
Indeed, formalizing proofs is notoriously difficult and only accessible to a handful of experts, which makes large annotation endeavours unrealistic~\cite{freek}.
To address data scarcity, previous work relies on large scale pretraining \cite{} or auxiliary tasks \cite{pact} to improve generalization. Other approaches use reinforcement learning \cite{} or expert iteration \cite{} to synthesize additional formal training data.

% although not lots of formal, lots of informal and impressive results in informal (minerva).
% in this paper, we propose to guide automated formal prover with informal proofs
Unlike formalized mathematics, informal data is abundant and widely available online.
In particular, large language models trained on a massive amount of mathetical web pages recently showcased impressive reasoning abilities~\cite{minerva}.
In this work, we explore two avenues to leverage informal data for the goal of producing formal proofs. Our methods hinge on so called proof sketches, which are high level sequences of reasoning steps written in a formal language, where each step is expected to be amenable to automatic proving. In this work, we focus on the Isabelle language and its powerful Sledgehammer~\cite{sledgehammer} for solving these intermediate steps. An example proof sketch is provided in Figure~\ref{fig:proof_skeleton}.

% declarative proofs and sledgehammer ? 

% say why not completely dumb setting
%  to produce a formal sketch
% given and used as-is
We consider the two settings where the informal proof is either an oracle proof (e.g. human-written), or generated by a large language model fine-tuned on mathematical data.
These two setups occur frequently when formalizing existing theories, where the informal proofs might be readily available, but also left to the reader or missing due to space limits in the margin.

% Note that t
% The first setup occurs frequently when formalizing existing theories with informal proofs readily available.
% following contributions

Our contributions are the following:
- First, we notice that with adequate prompting, along with an informal proofs of the targeted theorem, the \emph{Codex} model \cite{}, available through its public API, is able to produce good proof sketches, allowing to close XX\% of the theorems in the \miniff benchmark. To the best of our knowledge, the setting of formally closing a goal using an informal proof as conditioning has not been studied so far, despite its relevance to the communities currently formalising known theories. 
- Second, we leverage the reasoning capabilities and informal knowledge encoded in the \emph{Minerva} model to produce an informal proof for a given informal theorem. We can then use these informal proofs as conditioning for \emph{Codex}, thus removing the necessity for human-written informal proofs, but with a slightly lower accuracy of XX\% closed theorems. 







% % Whereas informal mathematical data is abundant enough to fine-tune a large language model, formalised proofs are scarce as they can only be written by a few experts. In this work, we explore two avenues to leverage informal data for the goal of producing formal proofs. Our methods hinge on so called proof-sketches, which are high level sequences of reasoning steps written in a formal language, where each step is expected to be amenable to automatic proving. In this work, we focus on the Isabelle language and its powerful Sledgehammer for solving these intermediate steps. An example proof sketch is provided in Figure~\ref{fig:proof_skeleton}.

% Unlike formalized mathematical data, informal data is abundant and widely available online. 
% In particular, large language models trained on a massive amount of math web pages recently showcased impressive reasoning abilities~\cite{minerva}.
% In this paper, we investigate a new setting where we leverage informal proofs (e.g. a proof written in Latex) to guide an automated theorem prover, by generating a formal \textit{proof sketch} with intermediate subgoals that follow the same reasoning steps as the informal proof (\autoref{fig:summary}).
% Intuitively, the proof sketch captures the global argument structure, reducing the proof to filling in local gaps.
% Our key idea is to use large-scale language models to generate these  proof sketches based on informal proofs,  offloading the task of filling in the gaps to a separate specialized system.
% % An example of informal proof with its corresponding proof skeleton is provided in Figure~\ref{fig:proof_skeleton}.





